Estimating the Distribution of Parameters in Differential Equations with Repeated Cross-Sectional Data

Differential equations are pivotal in modeling and understanding the dynamics of various systems, offering insights into their future states through parameter estimation fitted to time series data. In fields such as economy, politics, and biology, the observation data points in the time series are often independently obtained (i.e., Repeated Cross-Sectional (RCS) data). With RCS data, we found that traditional methods for parameter estimation in differential equations, such as using mean values of time trajectories or Gaussian Process-based trajectory generation, have limitations in estimating the shape of parameter distributions, often leading to a significant loss of data information. To address this issue, we introduce a novel method, Estimation of Parameter Distribution (EPD), providing accurate distribution of parameters without loss of data information. EPD operates in three main steps: generating synthetic time trajectories by randomly selecting observed values at each time point, estimating parameters of a differential equation that minimize the discrepancy between these trajectories and the true solution of the equation, and selecting the parameters depending on the scale of discrepancy. We then evaluated the performance of EPD across several models, including exponential growth, logistic population models, and target cell-limited models with delayed virus production, demonstrating its superiority in capturing the shape of parameter distributions. Furthermore, we applied EPD to real-world datasets, capturing various shapes of parameter distributions rather than a normal distribution. These results effectively address the heterogeneity within systems, marking a substantial progression in accurately modeling systems using RCS data.

==> backup <==
%\begin{tcbverbatimwrite}{tmp_\jobname_header.tex}
%\title{Estimating the Distribution of Parameters in Differential Equations with Repeated Cross-Sectional Data \LaTeX\ Style\thanks{Submitted to the editors.
%\funding{Hyung Ju Hwang was supported by the National Research Foundation of Korea(NRF) grant funded by the Korea government(MSIT) (No. RS-2023-00219980 and RS-2022-00165268) and by Institute for Information \& Communications Technology Promotion (IITP) grant funded by the Korea government(MSIP) (No.2019-0-01906, Artificial Intelligence Graduate School Program (POSTECH).}}}

%\author{Sung Woong Cho\thanks{Stochastic Analysis and Application Research Center, Korea Advanced Institute of Science and Technology, Daejeon 34141, Republic of Korea (\email{swcho95kr@kaist.as.kr}).}
%\and Hyeontae Jo\thanks{Department of Mathematics,  Korea University Sejong Campus, Sejong 30019, Republic of Korea (\email{korea_htj@korea.ac.kr}).}
%\and Hyung Ju Hwang\thanks{Department of Mathematics \& Graduate School of AI, Pohang University of Science and Technology (\email{hjhwang@postech.ac.kr}).}\footnotemark[3]}

% Custom SIAM macro to insert headers
%\headers{Estimating the Distribution of Parameters in Differential Equations with Repeated Cross-Sectional Data}{Sung Woong Cho, Hyeontae Jo, and Hyung Ju Hwang}
%\headers{Guide to Using  SIAM'S \LaTeX\ Style}{Dianne Doe, Paul T. Frank, and Jane E. Smith}

%\end{tcbverbatimwrite}




%\title{Estimating the Distribution of Parameters in Differential Equations with Repeated Cross-Sectional Data \thanks{Submitted to the editors DATE.}}
%\funding{Hyung Ju Hwang was supported by the National Research Foundation of Korea(NRF) grant funded by the Korea government(MSIT) (No. RS-2023-00219980 and RS-2022-00165268) and by Institute for Information \& Communications Technology Promotion (IITP) grant funded by the Korea government(MSIP) (No.2019-0-01906, Artificial Intelligence Graduate School Program (POSTECH) }

%\author{Sung Woong Cho\thanks{Stochastic Analysis and Application Research Center, Korea Advanced Institute of Science and Technology, Daejeon 34141, Republic of Korea (\email{ddoe@imag.com}).} \and Hyeontae Jo\thanks{Department of Mathematics,  Korea University Sejong Campus, Sejong 30019, Republic of Korea \email{korea_htj@korea.ac.kr}).} \and Hyung Ju Hwang \thanks{Department of Mathematics & Graduate School of AI, Pohang University of Science and Technology, ID \email{hjhwang@postech.ac.kr}).}\footnotemark[3]}

% Custom SIAM macro to insert headers
%\headers{Guide to Using  SIAM'S \LaTeX\ Style}{Sung Woong  Cho, Hyeontae Jo, and Hyung Ju Hwang}
%\input{tmp_\jobname_header.tex}

% Optional: Set up PDF title and authors
%\ifpdf
%\hypersetup{ pdftitle={Guide to Using  SIAM'S \LaTeX\ Style} }
%\fi

